Rectified Flow For Structure Based Drug Design

Deep generative models have achieved tremendous success in structure-based drug design in recent years, especially for generating 3D ligand molecules that bind to specific protein pocket. Notably, diffusion models have transformed ligand generation by providing exceptional quality and creativity. However, traditional diffusion models are restricted by their conventional learning objectives, which limit their broader applicability. In this work, we propose a new framework FlowSBDD, which is based on rectified flow model, allows us to flexibly incorporate additional loss to optimize specific target and introduce additional condition either as an extra input condition or replacing the initial Gaussian distribution. Extensive experiments on CrossDocked2020 show that our approach could achieve state-of-the-art performance on generating high-affinity molecules while maintaining proper molecular properties without specifically designing binding site, with up to -8.50 Avg. Vina Dock score and 75.0% Diversity.

==> tex/casestudy.tex <==
\section{Functional Annotator Failures in Detecting Functional Residues}
\qq{maybe change the section name to reflect the main findings of this section?}

\label{sec:case_study}
In this section, we aim to investigate the robustness of the existing state-of-the-art (SOTA) method, CLEAN \cite{yu2023clean}, with respect to protein functional tags and homologs. To evaluate its performance, we first demonstrate the F1 scores after adding protein tags, and also apply saliency detection techniques to CLEAN and observe instances where it may fail to adequately attend to crucial functional residues. This analysis provides insights into potential limitations of CLEAN and highlights the importance of addressing robustness issues in protein function prediction methodologies.

\paragraph{Protein Tagging and Homologous Proteins.}
In Table \ref{table:case_study:robustness}, we demonstrate that once appending functional tags or switching to homologous proteins, the CLEAN model cannot keep the same results. It first indicates that the CLEAN is not robust to these changes which do not change the protein functions due to human knowledge. It also suggests that the existing method does not really pay attention to functional residues and ignore the other residues. 

\begin{table*}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{l|cccccccc}
\toprule
 & \multicolumn{4}{c}{\new} & \multicolumn{4}{c}{\price} \\
\cmidrule(r){2-9}
Metric  & Original & His-Tag & HSV-Tag & Homolog & Original & His-Tag & HSV-Tag & Homolog\\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
F1 & 0.497 & 0.264 & 0.221& 0.405 & 0.495 & 0.168 & 0.130 & 0.412 \\
\% drop & 0\% & -- & -- & -- & 0\% & -- & -- & -- \\
\bottomrule
\end{tabular}}
\caption{
\textbf{CLEAN model is sensitive to common enzyme modifications encountered in protein engineering.} We demonstrate the drop in performance when modifying a protein sequence with common tags or replace it with a homolog. Here, His- (6mer) and HSV-tags (11mer) are common tags appended to the N- or C-terminus of proteins in molecular biology workflows.  Homolog indicates a homologous sequence with $\sim$80\% sequence similarity to the proteins in the test sets. `\% drop' demonstrates the difference from the results on the original test set.  \daiheng{here the tag I use is not His- (6mer) and HSV-tags (11mer), His-Tag is for 100H tag, HSV tag is for 10 times HSVhisMyc Mix(iterate)tag} \cygong{to do: let's modify and re-describe the settings a bit}
}
%  Enzyme Commission number classification F1 scores on \new and \price with different types of functional tags for the CLEAN \cite{yu2023clean} model.}
\label{table:case_study:robustness}
\end{table*}

\paragraph{Saliency Detection}
Therefore, we further apply self-supervised saliency detection with \cite{} \cygong{Class Activation Mapping?}. Upon testing on the MCSA labelled data, we observe that the detected residues do not consistently align with the labelled functional residues. \cygong{to do: pick two examples}
% \daiheng{the path is /data/daiheng/CLEAN/app/salience.py, I use chatgpt generate the salience map detection. Chengyue, please let me know if something need to be modified further.}

==> tex/method.tex <==
\section{Methods}
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/framework_v2.pdf}
    \caption{
    \textbf{Two-Stage Pipeline.}
    In the first stage, our model predicts which residues are functional.
    In the second stage, it pools these predicted functional residues to obtain a functional representation, which is decoded into an enzyme commission (EC) number prediction. \cygong{change the height / width ratio}
    }
    \lblfig{fig:main}
\end{figure}


\textbf{Overview of \nameshort.}
We propose a two-stage model for emzyme functional annotation. First, we train a functional residue classifier with MSA pseudo-labels that quantifies evolutionary 
conservation from MSA data \qq{what is this?
pseudo-labels that quantifies evolutionary 
conservation from MSA data? 
}. Then, based on the first model, we filter out non-functional residues and generate protein representation by weighted-averaging across the rest residues. Finally, we train the functional annotation model by doing multi-class classification. In this section, we first provide an overview of the two-stage model, followed by a detailed explanation of the training objectives for each stage.



\paragraph{Two Stage Pipeline.}
\qq{this and the last paragraphs feels a little repetitive. maybe make the last one more brief}
\qq{maybe formally introduce the two stages with two bullet points?}
As demonstrated in~\reffig{fig:main}, we propose a two-stage training pipeline for the functional annotation task.
We posit that protein function is closely associated with functional sites and residues. Consequently, our approach begins by identifying the functional residues within a protein. Previous studies \citep[e.g.][]{teukam2024language,derry2023collapse,derry2023parse} try to answer this question by self-supervised learning with MSA information. In our work, we propose to train a machine learning model to solve this problem with both labeled and pseudo-labeled data, which is generated from multiple sequence alignments (MSA).
\qq{have one or half sentence to explain what pseduo label mean here? say  both experimentally labeled data, and a set of pseudo-labels that we generate from multiple145 sequence alignments (MSA)? }.
Once the functional residues are identified, we utilize the confidence scores from the binary classification as weights. These weights are applied to the hidden representation of the top-k residues with the highest confidences. Subsequently, we employ a simple MLP network for EC number classification.


\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/msa_label_v2.pdf}
    \caption{
    \textbf{Generating pseudo-labels from multiple sequence alignments.}
    We introduce a self-supervised heuristic to extract functional residues from proteins using their MSAs.
    More specifically, residues in columns of low MSA entropy are identified as functional.
    \jz{histogram column names are too small. we can remove them or make them bigger}
    }
    \lblfig{msa}
\end{figure}

\paragraph{Functional Residue Identification with MSAs.}
We start from the functional residue classification model training. 
Denote the protein sequence as $P = \{a_i\}_{i=1}^n$ where $a_i$ indicates the amino acid at index $i$. With M-CSA Mechanism and Catalytic Site Atlas dataset, we have labelled data for every $a_i$ which indicates whether this amino acid is functional. We denote the labelled dataset $\mathcal{D}^\mathrm{sup} = \{ e_i, y_i\}$ \qq{what is the difference between $a_i$ and $e_i$? the same?} \cygong{$e_i$ is pass through the ESM model} whether $y_i \in \{0, 1\}$ is a binary label, and \qq{?}$e_i = \mathrm{ESM}(a_i)$ denotes the hidden representation of $a_i$ extracted from the pre-trained protein language model ESM \cite{}. In practice, we utilize the ESM model to extract representations, which can be substituted with those obtained from AlphaFold or other backbones. 

In addition to using labeled data, our model is trained with pseudo-labels generated from multiple sequence alignments (MSAs) (see \reffig{msa}).
Prior literature \cite[e.g.][]{cheng2005improvement, gong2024evolution, sturmfels2020profile} apply evolutionary conservation as the indicator of the location of functional sites. These pseudo-labels are generated based on the probability of amino acids being prone to mutation, as inferred from the MSAs.
we calculate the entropy of the following probability density function (\emph{p.d.f.}) 
derived from the MSA of the protein to detect the information, 
 \qq{maybe just  directly define entropy $\mathcal H_j$ and $p_j$ within a single equation. directly introduce the entropy.} 
%
\begin{equation} 
  p^\mathrm{MSA}_j(\ell) \propto 
  \sum_{ P'\in \text{MSA}(P)}
  \delta (\ell = \textbf{AA}(P', j)), 
  \label{eq:msa}
\end{equation}
%
where $\ell$ is one of the $20$ amino acids, $\delta$ is the delta function, $\textbf{AA}$ is the function to get the amino acid type at position $j$,
$\text{MSA}(P)$ denotes 
the set of sequences that are best aligned with $P$ 
via multiple sequence alignment on UniRef90 \citep{suzek2007uniref} with \cygong{software, and cite}. After getting the probability score for 20 amino acids at one position, we can calculate the entropy,
\begin{equation} 
  \mathcal{H}_j = - \sum_{\ell \in \mathcal{A} } p^\mathrm{MSA}_j(\ell) \log p^\mathrm{MSA}_j(\ell).
  \label{eq:entropy}
\end{equation}
\qq{should it be $\mathcal H_j$, per site?}
Here, $\mathcal{A}$ is the set of 20 amino acids. In practice, we calculate the entropy for all the positions in one protein sequence, and mark the top 10\% amino acids with the lowest entropy
as functional residues, and we mark the MSA labelled dataset as $\mathcal{D}^\mathrm{MSA} = \{e_i, y_i^\mathrm{MSA}\}$. 


To validate the reliability \qq{reliability?} of the pseudo-labels, we utilize the MCSA labeled dataset as a case study. By extracting all MSA files, computing entropy scores, and designating the lowest 10\% entropy residues in each sequence as functional, while considering the rest as non-functional, \cygong{we achieve a recall $0.5$, precision $0.1$ and F1 score $0.1$, while random prediction baseline gets recall $0.4$, precision $0.01$, F1 $0.02$.} \qq{is 0.5 high? also precision could be very low in principle?}. This outcome suggests that this straightforward criterion effectively identifies functional residues within a protein sequence. Additional findings and outcomes are detailed in our Experiment section.

With $\mathcal{D}^\mathrm{MSA}$ and $\mathcal{D}^\mathrm{sup}$, The loss function consists of two cross-entropy loss terms, one for labelled dataset and the other for the pseudo-label dataset. 
We propose to train the model with the following \cygong{confidence-aware} training objective. \qq{maybe highlight here that it is a "confidence aware" objective function? Write some motivation before introducing the equation, and then provide more justification as you did in the sequel.}
\begin{equation} 
  \mathbb{E}_{(e_i, y_i) \sim \mathcal{D}^\mathrm{sup}} \mathrm{CE}(q_f(e_i), y_i) + \lambda \mathbb{E}_{(e_i, y_i) \sim \mathcal{D}^\mathrm{MSA}} \mathbb{I}(\mathrm{max}( q_f(e_i) ) > \mathrm{Conf}) \mathrm{CE}(q_f(e_i), y_i),
  \label{eq:binary_loss}
\end{equation}
where $q_f(e_i)$ is the two-dimension predicted distribution generated by the model $f$, and $\mathrm{Conf}$ is a scalar hyperparameter which controls the confidence threshold.
In practice, we set $\mathrm{Conf} = 0.9$.
The first term on the MCSA dataset is the standard cross entropy loss, and the second term is a cross entropy loss with additional confidence threshold. 
% 
For each data instance, we ensure that our current trained model exhibits high confidence on the pseudo-label dataset. If the confidence level for a particular data instance is low, we discount the corresponding pseudo-label during gradient computation. Similar strategies have been employed in the past for disregarding low-confidence predictions in semi-supervised learning \cite{sohn2020fixmatch}, domain adaptation \cite{french2017self}, and other related problems where researchers utilize pseudo-labels. The rationale behind this approach is to ensure that the pseudo-label aligns with the training dataset, thereby enhancing the model's robustness and generalization ability. Since the model fits the training dataset, once we observes large disagreement, it indicates that the example may be different from the training dataset data points. 
\qq{the idea is not totally clear to me. For data with $q_f(e_i) > conf$, the confidence is already high, why do we need additional information (unless the pseudo label is not consistent with the experimental label, in which case it would lower the confidence?)? }

\qq{one may expect that the additioanal data is mostly useful for the un-confident data with $q_f(e_i) < conf$, but it is filtered out?} \cygong{the MSA dataset can be viewed as some data augmentation dataset, we select high-confidence augmentation, because the low-confidence data may be mis-labeled}

\paragraph{Protein Representations with Functional Residues.}
Once we get the model $q_f(\cdot)$ capable of discerning functional from non-functional residues, we proceed to embed a protein sequence $P = \{a_i, \cdots, a_n\}$ with sequence length $n$.

Utilizing the ESM embedding $e_i$ of each amino acid and the prediction $q_f(\cdot)$ we construct the protein sequence representation as follows, 
\begin{equation} 
  e(P) = \sum_{i=1}^n \mathbb{I}[ \pi(e_i) > \tau] \pi(e_i) e_i, ~~~~~\pi(e_i) = q_f(e_i; c=1),
  \label{eq:protein_embedding}
\end{equation}
\qq{$q_f(e_i; c=1)$ is strange. what is the definition? is not the filtering already done with $\tau$? do you mean something like $q_f \mathbb I(\max(q_f) >\tau)$?}
\cygong{after filtering out, we applying another weighted average, $q_f$ is the model outputs, we want to get the confidence score for the functional residue class}
where $\tau$ is a threshold hyperparameter dictating the number of amino acids considered in computing the protein embedding. The confidence score $\pi(e_i)$, derived from the binary classifier. Here, $c=1$ indicates that this residue class is functional.  Rather than employing average pooling or learnable attention layers, this approach leverages labelled functional residue data to directly obtain the protein embedding based on its functional residues.
In practice, we set $\tau$ to 80\% quantile for one given protein sequence.  

\paragraph{Functional Annotation Classification.}
With the protein functional representations in Eqn \eqref{eq:protein_embedding}, we train a classification model to solve the EC number classification problem. We encode each 4-digit EC number into one class, and train a 4096-way classification on the EC number dataset.  
We denote the dataset $\mathcal{D}^\mathrm{EC} = \{e(P_i), y_i^\mathrm{EC}\}$, and calculate the weighted cross entropy loss as the training objective, 
\begin{equation} 
  - \sum_{j=1}^{N} w_j^\alpha p\bigg( y_i^\mathrm{EC}\bigg) \log\bigg\{ q_g^j(e(P_i)) \bigg\}.
  \label{eq:ec_classification}
\end{equation}
Here, $N$ represents the number of EC classes, $w_j$ denotes the class weight generated based on class frequencies, and $\alpha$ is a hyperparameter controlling the weighting. For simplicity, we typically set $\alpha = 1$ in practice. 
% 
This loss function is employed due to the imbalanced nature of the EC number classes, and we observe that it establishes robust baselines comparable to or even surpassing the state-of-the-art method CLEAN \cite{yu2023clean}.


==> tex/result.tex <==
\section{Results}
\subsection{Experiment Details}
\myparagraph{Dataset}
We summarize the datasets used in this paper in~\reftbl{datasets}. We first introduce the functional residue identification datasets and MSA datasets we use, and then summarize the EC number classification training and test set details.

For supervised learning of the functional residues in a protein sequence, we use the Mechanism and Catalytic Site Atlas (mCSA~\cite{ribeiro2018mcsa}), a database of 820 protein sequences with 3716 annotated functional residues.
While mCSA provides mechanistic roles for the functional residues (e.g. general acid, transition-state stabilization, etc), we curate our dataset with functional residues as the positive class (2-10 residues per protein) and the remaining residues within a protein as the negative class.  

To evaluate our ability to identify functional residues, we split mCSA into a training set of 403 protein sequences with 1818 annotated residues and a validation set of 417 protein sequences with 1898 annotated residues.
To limit homology-based data leakage, proteins in the validation set are at most 50\% sequence similar to those in the training set.

For the EC number classification task, we use the training and test sets from CLEAN~\cite{yu2023clean}. Briefly, the training set consist of $220K$ enzyme sequences by clustering and subsampling SwissProt \cite{boeckmann2003swiss}, the human annotated subset of UniProtKB. 

For the EC number training dataset, the protein sequences in our training set are sampled from SwissProt \cite{boeckmann2003swiss}. It is a subset of the comprehensive UniProt dataset, which is meticulously reviewed by humans. This ensures that our model learns from human-curated annotations.  Adopting the data filtering methodology from CLEAN~\cite{yu2023clean}, we obtain a training set with around $220$K samples. To limit data-leakage with our test sets.  we cluster and subsample the data using MMSeqs2 using various sequence identity cutoffs at different thresholds (\emph{e.g.}, $10\%$, $30\%$), which helps limit homology-based data leakage \emph{w.r.t.} the test sets.

% The established test datasets are ($1$) \texttt{Price}, which contains $149$ test sequences; ($2$) \texttt{New}, which consists of $392$ enzymes sequences distributed across $177$ distinct EC numbers.
We evaluate our model's ability to predict EC numbers on the two established test datasets \new and \price.
The \new dataset, first introduced by CLEAN~\cite{yu2023clean}, contains $392$ enzyme sequences distributed across $177$ distinct EC numbers retrieved from Swiss-Prot.
The \price dataset, first introduced by ProteInfer~\cite{sanderson2023proteinfer}, consists of $149$ proteins~\cite{price2018mutant}.

\myparagraph{Hyperparameter Configurations}
Our experimental setup comprises a two-stage model for enzyme functional annotation. Initially, we train a functional residue classifier utilizing both labeled and pseudo-labeled data obtained from Multiple Sequence Alignments (MSAs). 
The model is a two-layer MLP with $256$ hidden dimension, and is trained with $10^{-5}$ learning rate, $0.01$ weight decay, $8192$ tokens in one iteration, and $10,000$ iterations with the AdamW optimizer. 
% 
We then train another three-layer MLP network with LayerNorm layers for EC number classification. We apply $4096$ hidden dimension, $4096$ batch size, $10^{-5}$ learning rate, $0.0$ weight decay, and $10,000$ iterations with the AdamW optimizer.
We apply $0.5$ label smoothing and mix-up data augmentation with $\alpha=0.2$. 

After pre-generating the ESM embedding for each sequences, the functional residue identification takes $\sim$15 minutes to train on a single A-40 GPU, while the EC number classification takes $\sim$10 minutes to train. 
The ESM embedding generation takes another 30 minutes on one A-40 single GPU.
% The entire training process takes $<1$ hour on a single $1$ A-40 GPU.

\myparagraph{Baselines}
We compare our model against a suite of computational and machine learning-based baselines.
Homology search has been the de-facto method for identifying an unknown function of a test protein.
BLASTp~\cite{altschul1990blast} retrieves previous labeled enzymes in the training set with high sequence similarity.
These homology search methods then assign the retrieved function as the predicted function for the test protein.
We implement this baseline following ProteInfer~\cite{sanderson2023proteinfer}.
COFACTOR~\cite{roy2012cofactor} performs homology search using structural similarity as opposed to sequence similarity.
Moreover, we compare to several machine learning-based baseline algorithms.
DeepEC~\cite{ryu2019deepec}, DEEPre~\citep{li2018deepre} and ECPred~\citep{dalkiran2018ecpred} classify an unknown protein with its EC number.
CLEAN~\citep{yu2023enzyme} and COLLAPSE~\cite{derry2023collapse} use self-supervised techniques to learn and leverage a functional latent space to label proteins.

\subsection{Enzyme Commission (EC) Classification}
We first demonstrate the results with 100\% data split in ~\reftbl{ec} on \new and \price datasets. We report traditional sequence alignemnt approaches in the firsst block, including BLAST and COFACTOR.
The middle block includes existing machine learning models such as COLLAPSE, ECPred, DeepEC, and CLEAN. 
The last block demonstrates our results. We observe that, by applying naive average pooling, our baseline results is already better than the SOTA on \new and comparable to the SOTA on \price. 
By applying our proposed protein functional representation, we further improve our baseline by 15\%, previous SOTA CLEAN by 33\% in the terms of F1 scores on \new. On Price, we improve the baseline by 7\%. 

In addition to showcasing the model performance on the main training dataset with a 100\% data split, we further analyze its effectiveness on alternative data splits (10\%,30\%, 50\%, 70\%) in ~\reftbl{data_split}.
The results for these additional data splits, along with more comprehensive metrics (macro and weighted F1 scores), are provided in the supplementary materials. This approach allows for a thorough examination of the model's performance across different training dataset configurations, providing insights into its robustness and generalization capabilities.

\begin{table*}[t]
\centering
\begin{tabular}{p{4cm}|ccc}
\toprule
Name & Annotation Type & Number of Proteins & Number of Categories \\
\cmidrule(r){1-4}
MSA (pseudo-label)& Functional Residue  & 19,000  & 2 \\
mCSA train~\cite{ribeiro2018mcsa} & Functional Residue & 403 & 2 \\
mCSA val~\cite{ribeiro2018mcsa} & Functional Residue & 417 & 2\\
\cmidrule(r){1-4}
CLEAN~\cite{yu2023clean} & EC Number & 220,000 & 4,096 \\
New-392~\cite{yu2023clean} & EC Number & 392  & 177 \\
Price-149~\cite{price2018mutant,sanderson2023proteinfer} & EC Number & 149 & 55 \\
\cmidrule(r){1-4}
\end{tabular}
\caption{
\textbf{Datasets}.
We leverage multiple datasets with varying levels of annotations.
For the mCSA residue function datasets, we treat any annotated residue as positive and all other residues as negative.
}
\lbltbl{datasets}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{\new} & \multicolumn{3}{c}{\price} \\
\cmidrule(r){2-7}
Model  & F1 & Prec & Rec  & F1 & Prec & Rec \\
\cmidrule(r){1-1}
\cmidrule(r){2-4}
\cmidrule(r){5-7}
BLAST~\cite{altschul1990blast} & - & - & - &  0.385 & 0.508 & 0.375 \\
COFACTOR~\cite{roy2012cofactor} & - & - & - & - & - & - \\
\cmidrule(r){1-1}
\cmidrule(r){2-4}
\cmidrule(r){5-7}
COLLAPSE~\cite{derry2023collapse}& - & - & - & - & - & -  \\
ECPred~\cite{dalkiran2018ecpred}& 0.100 & 0.118 & 0.095 & 0.020 & 0.020 & 0.020\\
DeepEC~\cite{ryu2019deepec}& 0.230 & 0.298 & 0.217 & 0.085 & 0.118 & 0.072 \\
CLEAN~\cite{yu2023clean} & 0.499 & 0.597 & 0.481 & 0.494 & 0.584 & 0.457 \\
\cmidrule(r){1-1}
\cmidrule(r){2-4}
\cmidrule(r){5-7}
MSA         & 0.582 & 0.629 & 0.568 & 0.493 & 0.565& 0.484 \\
Average Pooling     & 0.578 & 0.625 & 0.565 & 0.492 & 0.564 & 0.482 \\
\nameshort (Ours)   & \bf{0.644} & \bf{0.687} & \bf{0.636} & \bf{0.525} & \bf{0.592} & \bf{0.501} \\
\bottomrule
\end{tabular}
\caption{
\textbf{Enzyme Commission number classification on New-392 and Price-149.}
Top: traditional rule based approaches.
Middle: existing machine learning models.
Bottom: our model and relevant baselines.
COLLAPSE produces learned functional microenvironment representations using contrastive learning weighted by the MSA statistics.
We extract the embeddings using  \url{https://github.com/awfderry/COLLAPSE} and learn a one-hidden-layer small MLP for enzyme classification.
We report classification metrics at a sequence similarity split of 30\%.
BLAST~\cite{altschul1990blast} explore the space of enzymes given a starting enzyme.
COFACTOR~\cite{roy2012cofactor} additionally leverages structural homology to infer the EC number.
}
\lbltbl{ec}
\end{table*}


\begin{table*}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|cccccccc}
\toprule
 & \multicolumn{4}{c}{New-392} & \multicolumn{4}{c}{Price-149} \\
\cmidrule(r){2-9}
Model  & 10\% & 30\% & 50\% & 70\% & 10\% & 30\% & 50\% & 70\%\\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
CLEAN & 0.312 & 0.362 & 0.394 & 0.416 & 0.235 & 0.267 & 0.304 & 0.372\\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
\nameshort (Ours) & \bf{0.402} & \bf{0.447} & \bf{0.584} & \bf{0.605} & \bf{0.247} & \bf{0.284}& \bf{0.328}& \bf{0.399} \\
\bottomrule
\end{tabular}}
\caption{
\textbf{F1 scores on different data split settings.}  We demonstrate the model performance with different training datasets with different data splits. These datasets are generated due to different sequence similarity threshold as we demonstrated in the table.
}
\lbltbl{data_split}
\end{table*}



\begin{table*}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{l|cccccccccc}
\toprule
 & \multicolumn{5}{c}{\new} & \multicolumn{5}{c}{\price} \\
\cmidrule(r){2-11}
Model  & Orig & His-Tag & HSV-Tag & Nuc-Tag & Homo& Orig & His-Tag & HSV-Tag & Nuc-Tag & Homo \\
\cmidrule(r){1-1}
\cmidrule(r){2-6}
\cmidrule(r){7-11}
CLEAN & 0.497 & 0.264& 0.221& 0.477& 0.405 & 0.495 & 0.168& 0.130 &0.432 & 0.412 \\
\cmidrule(r){1-1}
\cmidrule(r){2-6}
\cmidrule(r){7-11}
Average Pooling & 0.578 & 0.327 & 0.288 & 0.557 & 0.513 & 0.492 & 0.171 & 0.128 & 0.433 & 0.409 \\
\nameshort (Ours) & \bf{0.644} & \bf{0.639} & \bf{0.636} & \bf{0.642} & \bf{0.632} & \bf{0.525} & \bf{0.521} & \bf{0.518} & \bf{0.522} & \bf{0.527}  \\
\bottomrule
\end{tabular}}
\caption{
\textbf{Enzyme Commission number classification on \new and \price.} with different types of adversarial noise. We report F1 scores and the changes compared to the clean data setting. $\Delta$ demonstrates the difference from the results on the original test set. We use the same settings in Section \ref{sec:case_study}.
\daiheng{https://docs.google.com/spreadsheets/d/1oGW2j91bSKX1Swn7czFlZlbZrVJEz8tr9W_nHXflGY0/edit?usp=sharing, save different tags here, please refer this}
}
\lbltbl{robustness}
\end{table*}

\subsection{Functional Residue Prediction}
We validate our model's ability to identify functional residues on the mCSA validation set.
This validation set has at most 50\% sequence similarity to the mCSA training set.
Here, function is defined as whether or not the residue is involved in the reaction.
We report binary classification metrics of F1, Precision and Recall in ~\reftbl{func}.

We compare against PROSITE~\cite{sigrist2012prosite} which finds functional residues by searching for expert curated sequence motifs (e.g. one amidation motif is ``x-G-[RK]-[RK]'').
In terms of machine learning models, we compare with PARSE~\cite{derry2023parse} which performs search in COLLAPSE's latent embedding and RXNAAMapper~\cite{teukam2024language} which correlates a language model's attention weights to a protein's binding site.
We also include an MSA statistics baseline that assigns the entropy of a residue in the MSA as the functional probability.

\name outperforms the traditional and machine learning-based methods, achieving $0.51$ F1 score, with the next best method at $0.44$.
Furthermore, we show that pre-training on the MSA significantly improves our model's ability to find functional residues, increasing our F1 score from $0.44$ to $0.51$.

\begin{table}[t]
\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace*{\fill}
\scalebox{0.9}{
\begin{tabular}{l|ccc}
\toprule
Model & F1 & Prec & Rec \\
\cmidrule(r){1-4}
Random & 0.020 & 0.011 & 0.445\\
PROSITE~\cite{sigrist2012new} & &  & \\
% UniRule~\cite{macdougall2020unirule}  &  &  &\\
\cmidrule(r){1-4}
RXNAAMapper ~\cite{teukam2024language} &  &  & \\
PARSE ~\cite{derry2023parse} &  &  & \\
\cmidrule(r){1-4}
MSA Statistics        & 0.101 & 0.094 & 0.502\\
\nameshort (w/o $\mathcal{D}^\mathrm{MSA}$)     & 0.442 & 0.516 & 0.393 \\
\nameshort (w/ $\mathcal{D}^\mathrm{MSA}$)     & \bf{0.510} & \bf{0.564} & \bf{0.442} \\
\bottomrule
\end{tabular}}
\caption{
\textbf{Functional residue prediction on mCSA validation set.}
We evaluate the model's ability to identify functional residues.
Our functional label is binary: either functional or not. Top: traditional rule based approaches. Middle: existing machine learning models. 
Bottom: our model and relevant baselines. Here, we split the training and test set due to 50\% sequence similarity to avoid data leakage.
% PROSITE (https://prosite.expasy.org/scanprosite/) is a bioinformatics tool that searches for functional motifs in protein sequences (akin to regular expressions).% PROSITE produces a list of active residue predictions.
}
\lbltbl{func}
\vspace*{\fill}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace*{\fill}
\scalebox{1.}{
\begin{tabular}{ccc|c}
\toprule
 Eqn \eqref{eq:ec_classification} & $\pi(e_i)$ & $\mathbb{I}[ p(e_i) > \tau]$ & F1  \\
\cmidrule(r){1-4}
\XSolidBrush & \XSolidBrush & \XSolidBrush & 0.304 \\
\cmidrule(r){1-4}
\checkmark & \XSolidBrush & \XSolidBrush & 0.578 \\
\checkmark & \checkmark & \XSolidBrush & 0.627 \\
\checkmark & \XSolidBrush & \checkmark & 0.604 \\
\cmidrule(r){1-4}
\checkmark & \checkmark & \checkmark & 0.644 \\
\bottomrule
\end{tabular}}
\caption{
\textbf{F1 scores on the \new dataset with different components.}  We demonstrate the model performance with difference techniques. Eqn \eqref{eq:ec_classification} is the class-imbalance-aware classification loss. $\pi(e_i)$ is the weighted function due to the binary classifier confidence. $\mathbb{I}[ p(e_i) > \tau]$ is the indicator function to filter out residues.
}
\lbltbl{ablation}
\vspace*{\fill}
\end{minipage}
\end{table}

\subsection{More Studies}
\paragraph{Robustness}
We demonstrate the model performance when applying augmentations in \reftbl{func}. We notice that, applying different types of functional types, out model still keep the same performance, while the CLEAN method cannot achieve the same results, because of the mean pooling layer in the architecture. While our method, on the other hand, achieve almost the same performance as the original dataset. In summary, \name is more robust than the existing SOTA method. 


\paragraph{Ablations}
We further demonstrate more ablation studies in \reftbl{ablation} to provide deeper understanding of different component in our method. 
We first notice that, applying the class imbalance loss contributes a lot to our baseline performance. With the class-imbalance loss shown in Eqn \eqref{eq:ec_classification}, we improve the F1 scores from 0.30 to 0.58. The other two techniques, applying confidence score as weighting function and filtering out unimportant residues, both contributes to the final performance. 
From the table, we observe a gradual increase in the F1 score as more components are incorporated into the model. When all components are included, the model achieves the highest F1 score of $0.644$. This indicates the importance of each component in contributing to the overall performance of the model.



\begin{table*}[htbp]

\end{table*}
% For the merge function, we demonstrate that different marge functions play a small difference. We further demonstrate that  



% \myparagraph{Merge function - topk sigmoid, softmax, temperature, normalization}

==> tex_final/casestudy.tex <==
\section{Robustness to Common Sequence Modifications} \dd{rewrote - Adam reformat}

\label{sec:case_study}
In this section, we demonstrate a drawback of CLEAN \cite{yu2023clean}, namely that it lacks robustness to sequence modifications that do not affect function (and therefore do not affect EC number).

% We evaluate the robustness of the existing state-of-the-art (SOTA) framework, CLEAN, to routine sequence modifications in experimental protein discovery and engineering. In molecular biology, tags are often added to the N- or C-terminus of a protein to improve expression, trigger secretion or localization to a cellular compartment, or enable purification and do not modify enzymatic function. During protein engineering, orthologs-- functionally related proteins that differ due to speciation-- are often screened in parallel to select a starting point to engineer. To evaluate CLEAN's robustness in these scenarios, we use the change in F1 scores after adding N-terminus protein tags and replacing with an orthologous sequence. Additionally, we apply saliency detection techniques to evaluate CLEAN's ability to adequately attend to crucial functional residues for EC number prediction. This analysis provides insight into the potential limitations of CLEAN and highlights the importance of developing ML frameworks robust to routine sequence augmentations in experimental protein discovery and engineering. 

% In this section, we aim to investigate the robustness of the existing state-of-the-art (SOTA) method, CLEAN \cite{yu2023clean}, with respect to protein functional tags and homologs. To evaluate its performance, we first demonstrate the F1 scores after adding protein tags, and also apply saliency detection techniques to CLEAN and observe instances where it may fail to adequately attend to crucial functional residues. This analysis provides insights into potential limitations of CLEAN and highlights the importance of addressing robustness issues in protein function prediction methodologies.

\paragraph{Evaluating Tags and Ortholog Sequence Augmentations} \dd {rewrote}
In Table \ref{table:case_study:robustness}, we demonstrate that the F1 score of the CLEAN framework is sensitive to N-terminus tags and replacement of an ortholog with $\sim$80\% sequence similarity to the proteins in \new and \price test sets. This sensitivity to non-functional sequence augmentations suggests that predictions by the CLEAN framework are not primarily driven by the functional residues within a protein, in particular catalytic residues. 




\paragraph{Saliency Detection} \dd {rewrote}
Therefore, we further apply self-supervised saliency detection using a discriminative localization technique \cite{zhou2016cam}. Using the mCSA database, we observe that CLEAN fails to  detect the experimentally validated functional residues of enzymes. We deduce that this insenstivity to functional residues is due to the average pooling layer used to obtain a fixed-length sequence representation in the CLEAN framework results in uniform attention over the entire sequence, shown in \lblfig{fig:saliency}. We notice that, for each protein sequence (each row), the saliency values are the same.
% 
In summary, we find that CLEAN's sensitivity to tag- or ortholog-based augmentated sequences is proportional to the extent of the sequence augmentation--longer tags and more divergent orthologs result in a larger F1 delta. 
% \daiheng{the path is /data/daiheng/CLEAN/app/salience.py, I use chatgpt generate the salience map detection. Chengyue, please let me know if something need to be modified further.}

==> tex_final/method.tex <==
\section{Methods}
\label{sec:method}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.92\columnwidth]{figs/framework_v2.pdf}
    \caption{
    \textbf{Overview of our two-stage EC number classification framework.}
    In the \textcolor{blue}{first stage}, our model predicts which residues are likely functional.
    In the \textcolor{brown}{second stage}, it pools these predicted functional residues to obtain a fixed-length function-aware representation, which is decoded into an enzyme commission (EC) number prediction using an MLP. 
    }
    \lblfig{fig:main}
    \vspace{-10pt}
\end{figure}


\textbf{Overview of \nameshort.} 
We propose a two-stage model for predicting enzyme function (EC number) from a protein sequence. First, we use semi-supervised learning to train a binary functional residue classifier with MSA pseudo-labels that quantifies evolutionary conservation from MSA data and the mCSA database as true functional residue labels. The binary classifier is used to filter non-functional residues and generate a fixed size representation from the predicted functional residue embeddings, which we call function-aware protein representations. Using function-aware protein representations, we train an EC number classification model. In this section, we provide an overview of the two-stage model and a detailed explanation of the training objectives for each stage.


\paragraph{Overview of the Two-stage Pipeline.}
% \qq{this and the last paragraphs feels a little repetitive. maybe make the last one more brief}
% \qq{maybe formally introduce the two stages with two bullet points?}
As demonstrated in~\reffig{fig:main}, we propose a two-stage training pipeline for the EC number classification task.
It is well established within the evolutionary biology community that a protein's function is executed by a select few functional residues and the primary goal of the structure is to provide a stable scaffold that correctly positions these residues in 3D space~\cite{cheng2005improvement,todd1999evolution}. Thus, our approach is based on identifying these functional residues in order to remove the remaining residues and generate a function-aware representation. Previous studies \citep[\emph{e.g.},][]{teukam2024language,derry2023collapse,derry2023parse} attempt to identify functional residues via self-supervised learning where labels are generated from the MSAs. In stage one of our work, we propose to expand experimentally characterized functional datasets with MSA-priors via semi-supervised learning to train a binary classifier. 
% pseudo-labels. train a machine learning model to solve this problem with both labeled and pseudo-labeled data, which is generated from multiple sequence alignments (MSA).
% \qq{have one or half sentence to explain what pseduo label mean here? say  both experimentally labeled data, and a set of pseudo-labels that we generate from multiple145 sequence alignments (MSA)? }.
To generate our function-aware representation, we utilize the confidence scores from the binary classifier to weight the hidden representation of the top-k most confident residues. In stage two of our work, we employ a simple MLP network to decode the function-aware representation into an EC number prediction, which we train via supervised learning.


\begin{figure}
    \centering
    \includegraphics[width=0.96\columnwidth]{figs/msa_label_v2.pdf}
    \caption{
    \textbf{Functional residue pseudo-label generation from multiple sequence alignments.}
    We introduce a self-supervised technique for labeling functionally relevant residues in a protein sequence from it's MSA.
    More specifically, conserved positions--10\% of columns with the lowest entropy--are labeled as functional.
    % \jz{histogram column names are too small. we can remove them or make them bigger}
    }
    \lblfig{msa}
    \vspace{-10pt}
\end{figure}

\paragraph{{Stage 1:} Functional Residue Identification with MSAs.}
We start by describing the functional residue classification model training. 
Denote the protein sequence as $P = \{a_i\}_{i=1}^n$ where $a_i \in \mathcal A$ indicates the amino acid at index $i$,
and  $\mathcal{A}$ is the set of 20 amino acids. 
In practice, we utilize the ESM model to extract representations, which can be substituted with those obtained from AlphaFold or other backbones. We note  the embedding by $\{ e_1, \cdots, e_n \} = \mathrm{ESM}(P)$, where $e_i$ denotes the contextualized hidden representation of $a_i$ extracted from the pre-trained protein language model ESM \cite{rives2019biological, lin2022language}.
% 
With the M-CSA (Mechanism and Catalytic Site Atlas) dataset, we have labeled data for every $a_i$ indicating whether this amino acid is functional. We denote the labelled dataset $\mathcal{D}^\mathrm{sup} = \{e_i, y_i\}$ 
where $y_i \in \{0, 1\}$ is a binary label and we collect all  amnio acid from all proteins. 

In addition to using labeled data from the mCSA database, our functional residue dataset is further augmented with pseudo-labels generated from multiple sequence alignments (MSAs) of CATH v4.3 \citep{sillitoe2021cath} (see \reffig{msa}).
% While prior literature \cite[\emph{e.g.},][]{cheng2005improvement, gong2024evolution, sturmfels2020profile} applies evolutionary conservation to identify functional sites, this alone is not sufficient to accurately discern functional residues from structurally important, non-functional residues. Thus, limiting their performance and generalization. 
To pseudo-label residues, we calculate the entropy of the following probability distribution derived from a protein's MSA as a proxy of evolutionary conservation of a site $a_i$: 
% are generated based on the probability of amino acids being prone to mutation, as inferred from the MSAs.
%
 % \qq{maybe just  directly define entropy $\mathcal H_j$ and $p_j$ within a single equation. directly introduce the entropy.} 
\begin{align} 
\begin{split}
  & %y_{i}^{\text{MSA}} =
  \mathcal{H}(p_i^{\text{MSA}}) \overset{\text{def}}{=}  - \sum_{a \in \mathcal{A} } p^\mathrm{MSA}_i(a) \log p^\mathrm{MSA}_i(a), \\ 
  & \text{with}~~~~~ p^\mathrm{MSA}_i(a) \propto 
  %\sum_{ P'\in \text{MSA}(P)}
  \sharp \{ P'\in \text{MSA}(P) \colon a = \textbf{AA}(P', i)\}, 
\end{split}  
  \label{eq:msa}
\end{align}
%
where $a \in \mathcal A$ is one of the $20$ amino acids, $\textbf{AA}$ is the function that outputs the amino acid type at position $i$,
$\text{MSA}(P)$ denotes 
the set of sequences that are best aligned with $P$ 
via multiple sequence alignment on UniRef90 \citep{suzek2007uniref}, and $\sharp\{\cdot\}$ denotes the number of elements of a set, and $\mathcal H(p)$ is the entropy function of distribution $p$.  
% After obtaining the probability score for the $20$ amino acids at one position, we can calculate the entropy
% \begin{equation} 
%   \mathcal{H}_j = - \sum_{\ell \in \mathcal{A} } p^\mathrm{MSA}_j(\ell) \log p^\mathrm{MSA}_j(\ell).
%   \label{eq:entropy}
% \end{equation}
% % \qq{should it be $\mathcal H_j$, per site?}
 %Here, $\mathcal{A}$ is the set of 20 amino acids. 
 
In practice, we calculate the entropy for all the positions $a_i$ in one protein sequence, and pseudo-label the top 10\% amino acids with the lowest entropy
as functional residues, and we pseudo-label the MSA labeled dataset as $\mathcal{D}^\mathrm{MSA} = \{e_i, y_i^\mathrm{MSA}\}$, where 
pseudo-label $y_i^\mathrm{MSA}= 1$
is positive for selected $10\%$ sites
and $y_i^\mathrm{MSA}= 0$ for the $90\%$ remaining sets. 
Because the size of the negative class ($y_i^\mathrm{MSA}= 0$) is $9$ times of that of the positive class, 
we resample the negative class to make the two classes  balanced. 


To validate the reliability of the pseudo-labels, we use the MCSA labeled dataset as a case study. By extracting all MSA files, computing entropy scores, and designating the lowest 10\% entropy residues in each sequence as functional, while considering the rest as non-functional, we achieve a recall of $0.5$, precision $0.1$ and F1 score $0.1$, while random prediction baseline gets recall $0.4$, precision $0.01$, F1 $0.02$. This outcome suggests that this straightforward criterion of a column in the MSA having low-entropy effectively identifies functional residues within a protein sequence. Additional findings and outcomes are detailed in Section \ref{sec:result}.

With $\mathcal{D}^\mathrm{sup}$ and $\mathcal{D}^\mathrm{MSA}$, one for labeled dataset and the other for the pseudo-label dataset, the loss function consists of two  logistic loss $\mathcal{L}$ terms. 
We propose to train the binary classifier $f$ with the following confidence-aware training objective,
% \qq{maybe highlight here that it is a "confidence aware" objective function? Write some motivation before introducing the equation, and then provide more justification as you did in the sequel.}
\begin{align} 
\begin{split}
  & \mathbb{E}_{(e_i, y_i) \sim \mathcal{D}^\mathrm{sup}} \left [\mathcal{L}
  \left(f(e_i), y_i\right) \right]
  +  
  \lambda \mathbb{E}_{(e_i, y_i^\mathrm{MSA}) \sim \mathcal{D}^\mathrm{MSA}} 
  \left [ w_i \mathcal{L}\left(f(e_i), y_i^\mathrm{MSA} \right)\right],
\end{split}
  \label{eq:binary_loss}
\end{align}
which is the sum of the standard cross entropy loss $\mathcal L_{CE}$ on the MCSA dataset $\mathcal D^{\text{sup}}$, 
and that of the MSA pseudo-labeled $\mathcal D^{\text{MSA}}$ 
weighted by additional confidence threshold $w_i$: 
\begin{align*}
  w_i =\mathbb{I}\left(\mathrm{max}( f(e_i), 1 - f(e_i) ) > \tau \right). 
\end{align*}
Here we assume that $f(e_i) \in [0, 1]$ is the output of the sigmoid gate,  and $\tau$ is a scalar hyperparameter which controls the confidence threshold $w_i$. 
In practice, we set $\tau = 0.9$ and $\lambda = 1$.


The intuition of the threshold $w_i$ is to ensure that, 
for each data instance,  our trained model exhibits high confidence on the pseudo-label that is used for training. If the confidence level for a particular data instance is low, we discount the corresponding pseudo-label during gradient computation. Similar strategies have been employed in the past for disregarding low-confidence predictions in semi-supervised learning \cite{sohn2020fixmatch}, domain adaptation \cite{french2017self}, and other related problems where researchers utilize pseudo-labels. 
%The rationale behind this approach is to ensure that
Doing this allows us to select the pseudo-labels that
aligns with the supervised dataset during training, thereby enhancing the model's robustness and generalization ability: 
the pseudo-labels that exhibit large disagreement with the MCSA labels  should be discarded to avoid potential harmful bias. 
%Since the model fits the training dataset, once we observes large disagreement, it indicates that the example may be different from the training dataset data points. 
% \qq{the idea is not totally clear to me. For data with $q_f(e_i) > conf$, the confidence is already high, why do we need additional information (unless the pseudo label is not consistent with the experimental label, in which case it would lower the confidence?)? }\qq{one may expect that the additioanal data is mostly useful for the un-confident data with $q_f(e_i) < conf$, but it is filtered out?} \cygong{the MSA dataset can be viewed as some data augmentation dataset, we select high-confidence augmentation, because the low-confidence data may be mis-labeled}

\paragraph{Stage 2a: 
Function-Aware Protein Representation.}
Given a learned model $f(\cdot)$, 
we  construct a representation of each protein $P$ by aggregation the information from their functional residuals as predicted by $f(\cdot)$.  
%With model $f(\cdot)$ in hand, we can describe our new protein sequence embedding. 

Let $P = \{a_i, \cdots, a_n\}$ be a protein with sequence length $n$, and the ESM embedding $e_i$ of each amino acid (recall these embeddings are contextualized by other amino acids in the sequence).
We construct the  function-aware representation of protein $P$
by a weighted sum of $e_i$: 
%is defined as 
%and the prediction $f(\cdot)$, we can construct our final protein sequence representation.
%We first apply the output confidence score $f(\cdot)$ together with a threshold $\tau$ \qq{used $\tau$ before, use a different notation here?} to filter out residues, and then use a weighting function $\omega$ to pay different attention to different residues.
%Concretely, the function-aware representation is defined as 
\begin{equation} 
  E(P) = \frac{1}{Z} \sum_{i=1}^n \omega_i  e_i,
  ~~~~~~~\omega_i = f(e_i) \mathbb{I}[ f(e_i) > \eta], 
  ~~~~~~~ Z = \sum_{i=1}^n \mathbb{I}[ f(e_i) > \eta ], 
  \label{eq:protein_embedding}
\end{equation}
where each $e_i$ is weighted by $\omega_i$ which is a thresholded variant of $f(e_i)$ that predicts whether $e_i$ is functional. 
The threshold $\eta$  is a hyperparameter dictating the number $Z$ of amino acids considered in computing the protein embedding. %, $Z$ is the number of amino acids selected based on $f(e_i) > \tau$.  
Instead of employing uniformly weighted average pooling or learnable attention layers, this approach leverages labeled functional residue data to directly obtain the protein embedding based on its functional residues.
In practice, %we apply $\omega(e_i) = f(e_i)$ and 
we set $\eta$ to 80\% quantile for one given protein sequence so that $Z = 80\% \times n$.   

\paragraph{Stage 2b: Functional Annotation Classification.} 
Using the function-aware protein representations in Eqn \eqref{eq:protein_embedding}, we train a classification model $g$ for the EC number classification task. We encode each 4-digit EC number into one class, and train a 4096-way classification head on the EC number dataset.  
We denote the dataset $\mathcal{D}^\mathrm{EC} = \{E(P_k), y_k^\mathrm{EC}\}$, where $k$ indexes the proteins in the dataset. 
Denote $\mathcal{L}_\mathrm{CE}$ as cross entropy loss, 
we use the weighted cross entropy loss as the training objective, 
\begin{equation} 
 \mathbb{E}_{\{E(P_k), y_k^\mathrm{EC}\} \sim \mathcal{D}^\mathrm{EC}} \left\{\phi(y_k^\mathrm{EC}) \mathcal{L}_\mathrm{CE}\left( g(E(P_k)), y_k^\mathrm{EC} \right ) \right\}.
  \label{eq:ec_classification}
\end{equation}
Here, $N$ represents the number of EC classes, $\phi(\cdot)$ weights each protein $P_k$ based on its EC class $y_k^{\text{EC}}$. 
In practice, we set $\phi$ as inverse the frequency of each class in the training set.
%
%This loss function is employed 
The weight $\phi(\cdot)$ is needed 
due to the imbalanced nature of the EC number classes, and we observe that it establishes a baseline comparable to the state-of-the-art method CLEAN \cite{yu2023clean}, while reducing the training cost by $\sim$80\%.
Compare to CLEAN's simple MLP network, we choose $g$ to be a three-layer MLP network, with layer normalization layers and a skip connection for the second layer. 


==> tex_final/result.tex <==

\begin{table*}[t]
\centering
\scalebox{0.94}{
\begin{tabular}{l|ccc}
\toprule
Dataset & Classification Task & Number of Proteins & Number of Classes \\
\cmidrule(r){1-4}
MSA & Functional Residue  & 19,000  & 2 \\
mCSA train~\cite{ribeiro2018mcsa} & Functional Residue & 403 & 2 \\
mCSA val~\cite{ribeiro2018mcsa} & Functional Residue & 417 & 2\\
\cmidrule(r){1-4}
CLEAN (100\% split)~\cite{yu2023clean} & EC Number & 220,000 & 4,096 \\
New-392~\cite{yu2023clean} & EC Number & 392  & 177 \\
Price-149~\cite{price2018mutant,sanderson2023proteinfer} & EC Number & 149 & 55 \\
\cmidrule(r){1-4}
\end{tabular}}
\caption{
\textbf{Datasets to train and evaluate the two stages of our framework}.
For each protein in the mCSA dataset, we label the annotated residues as positive and all other residues as negative. Similarly, to generate the MSA training dataset, the top 10\% of conserved residues of a protein are pseudo-labeled as positive, while the remaining 90\% are labeled as negative.
}
\lbltbl{datasets}
\end{table*}

\section{Results}
\label{sec:result}

\subsection{Experiment Details}
\myparagraph{Dataset} 
We summarize the datasets used in this paper in~\reftbl{datasets}. We first introduce the functional residue identification datasets and MSA datasets we use, and then summarize the EC number classification training and test set details.

For supervised learning of the functional residues in a protein sequence, we use the Mechanism and Catalytic Site Atlas (mCSA~\cite{ribeiro2018mcsa}), a database of 820 protein sequences with 3716 annotated functional residues.
While mCSA provides mechanistic roles for the functional residues (e.g. general acid, transition-state stabilization, etc), we curate our dataset with functional residues as positive class and the remaining residues as the negative class. 
% 
To evaluate our ability to identify functional residues, we split mCSA into a training set of 403 protein sequences with 1818 annotated residues and a validation set of 417 protein sequences with 1898 annotated residues. To limit homology-based data leakage, validation set proteins are at most 50\% sequence similar to those in the training set.

For the EC number classification task, we use the training and test sets from CLEAN~\cite{yu2023clean}. Briefly, the training set consist of $220K$ enzyme sequences by clustering and subsampling SwissProt \cite{boeckmann2003swiss}, the human-annotated subset of UniProtKB.
For evaluation, we use the \new and \price test sets. 
The \price dataset, introduced by ProteInfer~\cite{sanderson2023proteinfer}, consists of $149$ proteins~\cite{price2018mutant} across $55$ distinct EC numbers, including eight out-of-distribution (OOD) EC classes with respect to our training set.  
The \new dataset, introduced by CLEAN~\cite{yu2023clean}, is a more comprehensive benchmark, featuring $392$ enzyme sequences distributed across $177$ distinct EC numbers curated from Swiss-Prot.
Additionally, we evaluate the impact of removing homologous proteins from the training set with respect to the \price and \new test sets at various sequence identity cutoffs  (\emph{e.g.}, $10\%$, $30\%$,  $50\%$, $70\%$). These filtered training sets were originally introduced in CLEAN and obtained from their repository. 

\myparagraph{Hyperparameter Configurations} 
Our EC framework uses two-stage training procedure. 
In the first stage, we pre-generate ESM2 embeddings and train a residue-level binary classifier to identify functional residues using semi-supervised learning, where we use the mCSA dataset as positive true labels and low-entropy residues in the MSA dataset as positive pseudo-labels. The model is a two-layer MLP with $256$ hidden dimension, and is trained with $10^{-5}$ learning rate, $0.01$ weight decay, $8192$ tokens in one iteration, and $10,000$ iterations with the AdamW optimizer. 
In the second stage, we train a EC number classifier. This model is a three-layer MLP network with LayerNorm layers and a skip connection for the second layer,  $4096$ hidden dimension, $4096$ batch size, $10^{-5}$ learning rate, $0.0$ weight decay, and is trained for $10,000$ iterations using the AdamW optimizer. During training, we make use of label smoothing ($0.5$) and mix-up data augmentation ($\alpha=0.2$). 
Using one A-40 GPU, pre-generating the the ESM2 embedding requires $\sim$30 minutes, training the functional residue binary classifier requires $\sim$15 minutes, and training the EC classifier requires $\sim$10 minutes. 


\myparagraph{Baselines} 
We compare our model against a suite of computational and machine learning-based baselines.
Homology search has been the de-facto method to infer the function of a target protein lacking experimental validation.
BLASTp~\cite{altschul1990blast} retrieves previous labeled enzymes in the training set with high sequence similarity.
These homology search methods then assigns the retrieved function as the predicted function for the uncharacterized protein.
We implement this baseline following ProteInfer~\cite{sanderson2023proteinfer}.
% COFACTOR~\cite{roy2012cofactor} performs homology search using structural similarity as opposed to sequence similarity.
Moreover, we compare to several machine learning-based baseline algorithms.
DeepEC~\cite{ryu2019deepec}, EnzBERT~\cite{buton2023predicting} and ECPred~\citep{dalkiran2018ecpred} are classification frameworks for predicting the EC number. 
CLEAN~\citep{yu2023enzyme} is trained with contrastive learning where proteins with the same EC number are considered as positive pairs and pre-generated EC number cluster representation are used to conduct classifcation during inference.


\begin{table*}[t]
\centering
\scalebox{0.92}{
\begin{tabular}{l|cccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{\new} & \multicolumn{3}{c}{\price} \\
\cmidrule(r){2-7}
 & F1 $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$ & F1 $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$ \\
\cmidrule(r){1-1}
\cmidrule(r){2-4}
\cmidrule(r){5-7}
BLAST~\cite{altschul1990blast} & 0.442 & 0.523 & 0.422 &  0.385 & 0.508 & 0.375 \\
% COFACTOR~\cite{roy2012cofactor} & - & - & - & - & - & - \\
\cmidrule(r){1-1}
\cmidrule(r){2-4}
\cmidrule(r){5-7}
% COLLAPSE~\cite{derry2023collapse}& - & - & - & - & - & -  \\
ECPred~\cite{dalkiran2018ecpred}& 0.100 & 0.118 & 0.095 & 0.020 & 0.020 & 0.020\\
EnzBERT~\cite{buton2023predicting} & 0.153 & 0.220 & 0.134 & 0.04 1& 0.076 & 0.034 \\
DeepEC~\cite{ryu2019deepec}& 0.230 & 0.298 & 0.217 & 0.085 & 0.118 & 0.072 \\
ProteInfer~\cite{sanderson2023proteinfer} & 0.230 & 0.409 & 0.284 & 0.166 & 0.243 & 0.138 \\  
CLEAN~\cite{yu2023clean} & 0.497 & 0.597 & 0.481 & 0.494 & 0.584 & 0.457 \\
\cmidrule(r){1-1}
\cmidrule(r){2-4}
\cmidrule(r){5-7}
% MSA         & 0.582 & 0.629 & 0.568 & 0.493 & 0.565& 0.484 \\
% Naive baseline (Ours)     & 0.558 & 0.625 & 0.565 & 0.492 & 0.564 & 0.482 \\
\nameshort (Ours)   & \bf{0.644} & \bf{0.687} & \bf{0.636} & \bf{0.525} & \bf{0.592} & \bf{0.501} \\
\cmidrule(r){1-1}
\cmidrule(r){2-4}
\cmidrule(r){5-7}
SOTA Improvement   & 30\% & 15\% & 32\% & 6\% & 1\% & 10\% \\
\bottomrule
\end{tabular}}
\caption{
\textbf{Classification performance comparisons on the New-392 and Price-149 EC number test sets.}
Top: Sequence homology-based approach.
Middle: Literature machine learning frameworks.
Bottom: Our framework.
We report \name classification metrics using the complete CLEAN training set (100\% sequence similarity splits).
% COFACTOR~\cite{roy2012cofactor} additionally leverages structural homology to infer the EC number.
}
\lbltbl{ec}
\vspace{-10pt}
\end{table*}

\subsection{Enzyme Commission (EC) Number Classification} 
Here, we evaluate the second training stage: EC number classification using a function-aware protein representations.
We first demonstrate the results with 100\% sequence similarity data splits with respect to the \new and \price datasets (~\reftbl{ec}). In the first block, We report the traditional sequence alignment baseline, BLAST.
In the middle block, we report literature machine learning models, such as ECPred~\cite{dalkiran2018ecpred}, EnzBERT~\cite{buton2023predicting}, DeepEC~\cite{ryu2019deepec}, ProteinInfer~\cite{sanderson2023proteinfer}, and the recent SOTA method CLEAN~\cite{yu2023clean}. 
The last block demonstrates our results. 

With respect to F1 score, \name further improves over previous SOTA by 30\% on \new and $6\%$ on \price. We note that improvements on price is much more challenging due to to 15\% of the EC numbers in this test set lack training data and are out of distribution (OOD). To generalize to OOD EC number classes, we train an separate classification head to predict the  three-digit EC number (247-class classifier). In order to evaluate without inadvertently leaking whether a sequence belongs to an OOD EC number, we create a new classification head. This head selectively utilizes the Softmax neurons from either the four-digit or the three-digit EC number classification heads, depending on the availability of training data for a specific four-digit EC class. This post-training classification head enables a comprehensive assessment of the model's performance across various training dataset configurations, where the number of EC number classes lacking training data may vary. Additionally, it facilitates examination of the model's robustness and generalization capabilities.

In \reftbl{data_split}, we compare the generalization capability of CLEAN and \name using several homology-based data splits: 10\%,30\%, 50\%, 70\%.  \name outperforms CLEAN across the five data splits  with an average F1 performance improvement of $\sim$35\%. Notably, training \name with the 50\% sequence similarity filtered training set outperforms CLEAN trained with no homology filtering (100\% dataset) by 18\% (F1 0.584 vs 0.497). 

\begin{table*}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|cccccccccc}
\toprule
Test Dataset & \multicolumn{5}{c}{\new} & \multicolumn{5}{c}{\price} \\
\cmidrule(r){1-11}
\multirow{2}{*}{Dataset Size (K)}
& 10\% & 30\% & 50\% & 70\% & 100\% & 10\% & 30\% & 50\% & 70\% & 100\%\\
% \cmidrule(r){1-1}
\cmidrule(r){2-6}
\cmidrule(r){7-11}
 & 7.8 & 9.8 & 29.4 & 74.5 & 22.7 & 7.8 & 9.8 & 29.4 & 74.5 & 22.7\\ 
\cmidrule(r){1-1}
\cmidrule(r){2-6}
\cmidrule(r){7-11}
CLEAN & 0.312 & 0.362 & 0.394 & 0.416 & 0.497 & 0.235 & 0.267 & 0.304 & 0.372 & 0.495\\
\nameshort (Ours) & \bf{0.402} & \bf{0.447} & \bf{0.584} & \bf{0.605} & \bf{0.644} & \bf{0.247} & \bf{0.284}& \bf{0.328}& \bf{0.399} & \bf{0.525}\\
\cmidrule(r){1-1}
\cmidrule(r){2-6}
\cmidrule(r){7-11}
Improvement & 29\% & 23\% & 48\% & 45\% & 30\% & 5\% & 6\% & 8\% & 7\% & 6\% \\
\bottomrule
\end{tabular}}
\caption{
\textbf{F1 scores on different homology-based data split settings.}  We evaluate performance on the \new and \price test sets when trained at different homology-filtering thresholds. These homology-filtered datasets are provided by CLEAN.
}
\lbltbl{data_split}
\vspace{-10pt}
\end{table*}



\begin{table*}[th]
\centering
\scalebox{0.82}{
\begin{tabular}{l|cccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{4}{c}{\new} & \multicolumn{4}{c}{\price} \\
\cmidrule(r){2-9}
& Original & Halo-Tag & TAP-Tag & Ortholog & Original & Halo-Tag & TAP-Tag & Ortholog\\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
CLEAN $\uparrow$ & 0.497 & 0.302 & 0.434 & 0.405 & 0.495 & 0.190 & 0.342 & 0.412 \\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
CLEAN sensitivity $\downarrow$ & 0\% & 39\% & 13\% & 19\% & 0\% & 62\% & 31\% & 17\% \\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
% naive-baseline (Ours) & 0.578 & 0.327 & 0.288  & 0.513 & 0.492 & 0.171 & 0.128 & 0.409 \\
\nameshort (Ours) $\uparrow$ & \bf{0.644} & \bf{0.619} & \bf{0.632} & \bf{0.632} & \bf{0.525} & \bf{0.503} & \bf{0.512} & \bf{0.527}  \\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
\nameshort sensitivity $\downarrow$ & 0\% & 4\% & 2\% & 2\% & 0\% & 4\% & 3\% & 0\% \\
\cmidrule(r){1-1}
\cmidrule(r){2-5}
\cmidrule(r){6-9}
Improvement $\uparrow$ & 30\% & 105\% & 46\% & 56\% & 6\% & 165\% & 50\% & 28\%  \\
\bottomrule
\end{tabular}}
\caption{
\textbf{Robustness comparisons on the \new and \price test sets using bio-based sequence modifications.} We report F1 scores under various sequence modification settings. `Sensitivity' demonstrates the difference between the results on the original test set and on the augmented test set as a percentage. 
`Improvement' demonstrates the difference in F1 performance between CLEAN and \name.
We use the same settings presented in \reftbl{table:case_study:robustness}. 
}
\lbltbl{robustness}
\end{table*}

\begin{table}[htbp]
\centering
\scalebox{0.85}{
\begin{tabular}{l|c|cccc}
\toprule
Metric & CLEAN & ESM-1b & ESM2-35M  & ESM2-650M & ESM2-3B  \\
\cmidrule(r){1-6}
F1 $\uparrow$ & 0.497 & \bf{0.644} & 0.580 & 0.626 & 0.629 \\
\cmidrule(r){1-6}
Precision $\uparrow$ & 0.597 & \bf{0.687} & 0.616 & 0.660 & 0.663\\
Recall $\uparrow$ & 0.481& \bf{0.636} & 0.578 & 0.631 & 0.631 \\
\bottomrule
\end{tabular}}
\vspace{5pt}
\caption{
\textbf{Metrics on the \new dataset using different backbones.} We evaluate the impact different ESM-based backbones have on the EC number classification task.
}
\lbltbl{ablation}
\end{table}

\paragraph{Robustness to Bio-based Sequence Modifications}
In protein engineering workflows, protein sequences are frequently modified with functional tags or screened alongside homologs. Therefore, it is crucial for EC number predictions to be robust to such modifications, since they generally don't alter enzymatic function.
Building upon the case study presented in the introduction (\reftbl{table:case_study:robustness}), we compare the model performance of \name vs CLEAN in these scenarios, using two N-terminus tags and orthologs with an $\sim$80\% sequence similarity, as shown in \reftbl{func}. For all sequence modification experiments on \price and \new, our method consistently exhibits superior robustness compare to CLEAN. We attribute this enhanced robustness to our function-aware representations, in contrast to CLEAN's, which derives its representation through average pooling.



\begin{table}[t]
% \begin{minipage}[t]{0.48\textwidth}
\centering
% \vspace*{\fill}
\scalebox{.88}{
\begin{tabular}{l|ccc|c}
\toprule
Model & F1 $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$ & EC Classification F1 $\uparrow$\\
\cmidrule(r){1-5}
Random & 0.020 & 0.011 & 0.445 & 0.482 \\
% PROSITE~\cite{sigrist2012new} & &  & \\
% UniRule~\cite{macdougall2020unirule}  &  &  &\\
% \cmidrule(r){1-4}
% RXNAAMapper ~\cite{teukam2024language} &  &  & \\
% PARSE ~\cite{derry2023parse} &  &  & \\
% \cmidrule(r){1-5}
MSA & 0.101 & 0.094 & 0.502 & 0.582 \\
\nameshort (w/o $\mathcal{D}^\mathrm{MSA}$)     & 0.442 & 0.516 & 0.393 & 0.612 \\
\nameshort (w/ $\mathcal{D}^\mathrm{MSA}$)     & \bf{0.510} & \bf{0.564} & \bf{0.442} & \bf{0.644} \\
\bottomrule
\end{tabular}}
\vspace{5pt}
\caption{
\textbf{Functional residue prediction on mCSA validation set.} 
We evaluate the binary classifier's performance on identifying functional residues.
MSA denotes applying low-entropy policy to distinguish functional residues.
Here, we split the training and test set due to 50\% sequence similarity to avoid data leakage.
The last column provides downstream evaluations on the \new test set.
% PROSITE (https://prosite.expasy.org/scanprosite/) is a bioinformatics tool that searches for functional motifs in protein sequences (akin to regular expressions).% PROSITE produces a list of active residue predictions.
}
\vspace{-5pt}
\lbltbl{func}
% \vspace*{\fill}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \vspace*{\fill}
% \scalebox{1.}{
% \begin{tabular}{ccc|c}
% \toprule
%  Eqn \eqref{eq:ec_classification} & $\pi(e_i)$ & $\mathbb{I}[ p(e_i) > \tau]$ & F1  \\
% \cmidrule(r){1-4}
% \XSolidBrush & \XSolidBrush & \XSolidBrush & 0.304 \\
% \cmidrule(r){1-4}
% \checkmark & \XSolidBrush & \XSolidBrush & 0.578 \\
% \checkmark & \checkmark & \XSolidBrush & 0.627 \\
% \checkmark & \XSolidBrush & \checkmark & 0.604 \\
% \cmidrule(r){1-4}
% \checkmark & \checkmark & \checkmark & 0.644 \\
% \bottomrule
% \end{tabular}}
% \caption{
% \textbf{F1 scores on the \new dataset with different components.}  We demonstrate the model performance with difference techniques. Eqn \eqref{eq:ec_classification} is the class-imbalance-aware classification loss. $\pi(e_i)$ is the weighted function due to the binary classifier confidence. $\mathbb{I}[ p(e_i) > \tau]$ is the indicator function to filter out residues.
% }
% \lbltbl{ablation}
% \vspace*{\fill}
% \end{minipage}
\end{table}



\paragraph{Backbone Ablations} 
In \reftbl{ablation}, we conduct an ablation study to compare the ESM-1b \cite{rives2019biological} backbone against three ESM2 backbones (\emph{e.g.}, 35M, 650M, 3B).
ESM-1b serves as the backbone for both our literature transformer-based baseline studies and the backbone of \name{}. Through ablation studies, we find that the specific choice of backbone has minimal impact, while the size of the backbone plays a more crucial role.
ESM-1b is the backbone used by our literature transformer-based baseline studies and is the backbone \name{} is built with. From these ablations studies, we observe that the backbone does not have a significant impact but rather the size of the backbone is much more important. 
Once we apply a larger backbone, \emph{e.g.,} ESM2 3B, ESM2 650M, the fluctuation in performance is not significant and can likely be mitigated through hyperparameter tuning. Remarkably, despite the ESM2 35M backbone being 18.6 times smaller than CLEAN's backbone, \name still achieves an F1 score that surpasses CLEAN by $\sim$17\%  (0.58 vs 0.497). This highlights the effectiveness of learning function-aware protein representations. 


% for different model backbones. First, ESM-1b \cite{rives2019biological} which is used in most of the previous studies and as the default backbone model in our work. Second, we apply different scale ESM2 models (\emph{e.g.}, 35M, 650M, 3B) to have a understanding of the backbone impacts.
% From \reftbl{ablation}, we notice that all the models get good performance. ESM2 35M model gets the worst performance, since the model is not large enough to learn enough meaningful information during pre-training. Once we apply a large backbone, \emph{e.g.,} ESM2 3B, ESM2 650M, the performance does not have significant difference. 


\subsection{Functional Residue Classification}
In this section, we assess the initial training stage, which involves a binary classifier aimed at identifying functional residues within a protein sequence via semi-supervised learning. 
For this evaluation, we split the mCSA dataset into a training and validation set using a 50\% sequence similarity threshold. 
We report binary classification metrics of F1, Precision and Recall in ~\reftbl{func}.
% 
We compare against the following baselines: a random classifier, our low-entropy MSA policy for pseudo-labeling residues, and supervised learning with the mCSA training set. 
The low-entropy MSA baseline shows that MSA conservation alone is inadequate for accurately distinguishing functional residues from structurally conserved positions, resulting in low precision. However, when combined with mCSA for semi-supervised learning, it boosts the F1 score from $0.44$ to $0.51$, marking a 15.4\% improvement, and enhances the downstream EC classification F1 score by 5.2\%. This underscores the effectiveness of our representations in improving performance on downstream functional tasks.



% The first is a random classifier which labels half of the position as functional residues. The other is the low-entropy position policy on the MSA where we pseudo-label the  10\% most conserved residues within a protein as functional residues. 
% PROSITE~\cite{sigrist2012prosite} which finds functional residues by searching for expert curated sequence motifs (e.g. one amidation motif is ``x-G-[RK]-[RK]'').
% In terms of machine learning models, we compare with PARSE~\cite{derry2023parse} which performs search in COLLAPSE's latent embedding and RXNAAMapper~\cite{teukam2024language} which correlates a language model's attention weights to a protein's binding site.
% We also include an low-entropy MSA baseline where we label the  10\% most conserved residues within a protein as functional residues. 
 




\iffalse
From these ablation studies, we observe that the class imbalance loss has significant impact; the class-imbalance loss (shown in Eqn \eqref{eq:ec_classification}) improves the F1 score from 0.30 to 0.58, a 93\% improvement. Our two bio-inspired techniques, weighting residues based on their functional residue score and filtering non-functional residues both make meaningful contribution to performance. 
These two techniques independently improve the F1 score by 8.5\% and 4.5\% to 0.627 and 0.608, respectively. When both bio-inspired techniques are combined, the model achieves the highest F1 score of $0.644$, an 11.4\% improvement over the class imbalance baseline. Thus, each component of our method makes a meaningful contribution. Overall, compared the naive-baseline with an F1 score of 0.304, our method improves the F1 score by 112\%. 
\fi




\begin{table*}[htbp]

\end{table*}
% For the merge function, we demonstrate that different marge functions play a small difference. We further demonstrate that  



% \myparagraph{Merge function - topk sigmoid, softmax, temperature, normalization}
